On the Power of Pre-training for Generalization in RL: Provable Benefits and Hardness

Generalization in Reinforcement Learning (RL) aims to learn an agent during training that generalizes to the target environment. This paper studies RL generalization from a theoretical aspect: how much can we expect pre-training over training environments to be helpful? When the interaction with the target environment is not allowed, we certify that the best we can obtain is a near-optimal policy in an average sense, and we design an algorithm that achieves this goal. Furthermore, when the agent is allowed to interact with the target environment, we give a surprising result showing that asymptotically, the improvement from pre-training is at most a constant factor. On the other hand, in the non-asymptotic regime, we design an efficient algorithm and prove a distribution-based regret bound in the target environment that is independent of the state-action space.

==> content/proof_useful.tex <==
\section{Omitted details for Section~\ref{sec: fine-tuning upper bound}}
\label{appendix_proof_usefel}
\subsection{Properties of the Set Returned in the Pre-train Stage}
We first show that the set $\hat \caU$ returned by the pre-train stage satisfies some properties that are needed in the test stage.
Recall that $\caU^* $ is the minimum set of MDPs with $\caP(\caU^*) \geq 1 - \delta$.
For simplicity, for each round $T$, we let $\hat \caP_T(\caU)$ to denote $\sum_{\M \in \caU} \frac{N_\M}{T}$, and let $T_0$ to denote $\lceil \frac{2|\caU^*|^2}{\delta^2} \log \frac{M}{\delta} \rceil$.

\begin{lemma}
\label{lemma_pretrain}
With probability at least $1 - 2\delta$, Alg.~\ref{alg: optimistic posterior fine-tuning} can return $\hat \caU$ with at most $T_0$ MDP samples in the pre-train stage such that $\mathcal P(\hat \caU) \geq 1 - 4\delta, |\hat \caU |\leq|\caU^*| $.
\end{lemma}


To prove Lemma~\ref{lemma_pretrain}, we first state the following high-probability events.
\begin{lemma}
\label{lemma_gap_star}
With probability at least $1-\delta$, for all $ T \in [\frac{4\log \frac M \delta}{\delta^2}, T_0]$, we have $|\mathcal P(\caU^*) - \hat {\caP}_T(\caU^*)| < \delta$.
\end{lemma}
\begin{proof}
Notice that $\caU^*$ is a fixed set. For any fixed $T \in [\frac{4\log \frac M \delta}{\delta^2}, T_0]$, with probability at least $1-\frac {\delta}{T_0}$, we have 
$$
|\mathcal P(\caU^*) - \hat {\caP}_T(\caU^*)| \leq \sqrt{\frac{\log \frac{T_0}{\delta}}{T}} < \delta \cdot \sqrt{\frac{4 \log \frac M \delta}{4 \log \frac M \delta}} = \delta.
$$
The proof is finished by taking union bound for all $T \in  [\frac{4\log \frac M \delta}{\delta^2}, T_0]$.
\end{proof}

\begin{lemma}
\label{lemma_gap_estimation}
With probability at least $1-\delta$, for all $ T \in [\frac{4\log \frac M \delta}{\delta^2}, T_0]$ such that $T > 2\frac{|\hat \caU_T|^2}{\delta^2}\log \frac M \delta$, we have $|\caP(\hat \caU_T) - \hat \caP_T(\hat \caU_T)|<2\delta$.
\end{lemma}
\begin{proof}
For any fixed $T, \M \in \Omega$, with probability at least $1 - \frac{\delta}{MT_0}$, we have 
$$
|\frac{N_\M}{T} - p_\M| \leq \sqrt{\frac{\log \frac {MT_0}{\delta}}{T}}.
$$
By union bound, with probability at least $1-\delta$, this is true for all $T \in [\frac{4\log \frac M \delta}{\delta^2}, T_0], \M \in \Omega$.

Conditioned on this, when $T >  2\frac{|\hat \caU_T|^2}{\delta^2}\log \frac M \delta$, we have
$$
|\caP(\hat \caU_T) - \hat \caP_T(\hat \caU_T) | \leq \sum_{\M \in \caU_T} |\frac{N_\M}{T} - p_\M| \leq |\caU_T| \sqrt{\frac{\log \frac {MT_0}{\delta}}{T}} \leq \delta \cdot \sqrt{\frac{\log \frac {MT_0}{\delta}}{2\log \frac M \delta}} < 2\delta.
$$
\end{proof}

Now we are ready to prove Lemma~\ref{lemma_pretrain}.
\begin{proof}
(Proof of Lemma~\ref{lemma_pretrain}) With probability at least $1-2\delta$, the statements in Lemma~\ref{lemma_gap_star} and \ref{lemma_gap_estimation} hold.
% For all $T, |\hat \caU_T| \geq 1$, the algorithm can never return when $T < \frac{2 \log \frac M \delta}{\delta^2}$.
Conditioned on this, for all $T \in [\frac{4\log {\frac M \delta}}{\delta^2}, T_0]$, we have $\hat \caP_T (\caU^*) > \caP (\caU^*)   - \delta \geq 1 - 2\delta$. 
According to the minimum of the selection process, $|\hat \caU_T|  \leq |\caU^*|$. So when $T = T_0 $, the return condition $T \geq \frac{2|\hat \caU_T |^2}{\delta^2}\log \frac M \delta$ is satisfied. We thus prove that the algorithm must return when $T \in [\frac{4\log \frac M \delta}{\delta^2}, T_0]$, and upon return, $|\hat \caU_T|  \leq |\caU^*|$.

In addition, according to Lemma~\ref{lemma_gap_estimation}, upon return, we have $|\caP(\hat \caU_T) - \hat \caP_T(\hat \caU_T)| < 2\delta$. Since $\hat \caU_T$ is selected such that $ \hat \caP_T(\hat \caU_T) > 1-2\delta$, we have $\caP(\hat \caU_T)  \geq 1 - 4\delta$.
\end{proof}

\subsection{Proof of Theorem~\ref{theorem_useful_restate}}
In Lemma~\ref{lemma_pretrain}, we prove that the MDP set $\hat{\caU}$ returned in the pre-training stage satisfies $\caP(\hat{\caU}) \geq 1-4 \delta$ with probability at least $1-2\delta$. Note that this event happens with high probability. If this event does not happen (w.p. $2\delta$), the regret can still be upper bounded by $K$, which leads to an additional term of $K \cdot 2\delta = 2\sqrt{K}$ in the final bound. This term is negligible compared with the dominant term in the regret. In the following analysis, we only discuss the case where the statement in Lemma~\ref{lemma_pretrain} holds.

We use $L$ to denote the maximum epoch counter, which satisfies $L \leq |\hat{\caU}|$. Note that under the event defined in Lemma~\ref{lemma_pretrain} $\caM^* \in \hat{\caU}$ with probability at least $1-4\delta$. In the following proof, we also assume $\caM^* \in \caU$ holds. If this condition is violated, the regret can still be upper bounded by $K$, which leads to an additional term of $K \cdot 4\delta = 4\sqrt{K}$ in the final bound. This will also not influence the main term in the regret bound.  
\begin{lemma}
\label{lemma: optimism, fine-tuning}
(Optimism) With probability at least $1-\delta/2$, we have $V^{*}_{\M^l,1}(s_1) \geq V^*_{\M^*,1}(s_1), \forall l \in [L]$.
\end{lemma}

\begin{proof}
To prove the lemma, we need to show that $\M^*$ will never be eliminated from the set $\caU_l$ with high probability. Condition on the sampled $\M^*$, for a fixed episode $k \in [K]$, by Azuma's inequality, we have:
\begin{align}
    \mbP\left(|{O}_{k,\M^*} - \hat{O}_k| \geq \sqrt{2H(k-k_0)\log(4K/\delta)}\right) \leq \delta/(2K).
\end{align}
By union bound over all $k \in [K]$, we know that
\begin{align}
    \label{inq: exclusive event}
    &\mbP\left(\exists k \in [K], |{O}_{k,\M^*} - \hat{O}_k| \geq  \sqrt{2H(k-k_0)\log(4K/\delta)}\right)
    \leq  \delta/2
\end{align}

%Inq.~\ref{inq: exclusive event} is exclusive with the event defined in $o_{k,i}$. Therefore, we know that the probability that $\M^*$ is eliminated from the instance set is at most $K \sum_{i=1}^{M}\delta_{\M_i,\M^*}$
\iffalse
Note that the above discussion is conditioned on a sampled $\M^*$ from the prior distribution $D$. Therefore, we can calculate the probability that $\M^*$ is eliminated from the instance set by summing over all possible $\M^* \in \Omega$.  That is
\begin{align}
    \label{inq: elimination prob 2}
    \sum_{j=1}^{M} p_{j} K \sum_{i=1}^{M}\delta_{\M_i,\M_j} = &  \frac{1}{4M}\sum_{j=1}^{M}p_{j} \sum_{i=1}^{M} \frac{p_i\delta}{(1-\delta)p_j + \delta p_i} \\
    \leq & \frac{1}{4M}\sum_{j=1}^{M}  \sum_{i=1}^{M} p_{i} p_{j} \delta\max\left\{ \frac{1}{p_i}, \frac{1}{p_j}\right\} \\
    \leq & \frac{1}{4M}\sum_{j=1}^{M} \sum_{i=1}^{M} p_{i} p_{j} \delta\left( \frac{1}{p_i}+\frac{1}{p_j}\right) \\
    \leq & \delta/2.
\end{align}
\fi
Therefore, $\M^*$ will never be eliminated from the set $\caU_l$ with probability at least $1-\delta/2$. By the definition that $V^*_{\M^l,1}(s_1) = \max_{\M \in \caU_k}V^*_{\M,1}(s_1)$, we have $V^*_{\M^l,1}(s_1) \geq V^*_{\M^*,1}(s_1)$.

\end{proof}

Now we are ready to prove Theorem~\ref{theorem_useful_restate}.
\begin{proof}
We use $\tau_{l}$ to denote the starting episode of epoch $l$. Without loss of generality, we set $\tau_{L+1} = K+1$.

By lemma~\ref{lemma: optimism, fine-tuning}, we know that $V^*_{\M^l,1}(s_1) \geq V^*_{\M^*,1}(s_1)$ with high probability. Under this event, we can decompose the value gap recursively following the standard decomposition techniques:
\begin{align}
    & \sum_{k=1}^{k} \left( V^*_{\caM^*,1}(s_1) - V^{\pi_k}_{\caM^*,1}(s_1)\right) \\
    \leq & \sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \left( V^*_{\M^l,1}(s_1) - V^{\pi_k}_{\caM^*,1}(s_1)\right) \\
    \label{inq: regret part 1, fine-tuning}
    \leq & \sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(R_{\M^l,h}(s_{k,h},a_{k,h}) + \mbP_{\M^l,h}V^*_{\M^l,h+1}(s_{k,h},a_{k,h}) - r_{k,h} - V^*_{\M^l,h}(s_{k,h+1})\right) \\
    \label{inq: Martingle 1, fine-tuning}
    & + \sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(r_{k,h} - R_{\M^*,h}(s_{k,h},a_{k,h})\right) \\
     \label{inq: Martingle 2, fine-tuning}
    & + \sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(V^{\pi_k}_{\M^*,h+1}(s_{k,h+1})-\mbP_{\M^*,h}V^{\pi_k}_{\M^*,h+1}(s_{k,h},a_{k,h})\right).
\end{align}
Note that $V^*_{\M^l,1}(s)$ is the value function of policy $\pi_k$ on MDP $\M^l$ if $\tau_l \leq k \leq \tau_{l+1}-1$. The second inequality is derived recursively from the following inequality:
\begin{align*}
    &V^{*}_{\M^l,h}(s_{k,h}) - V^{\pi_k}_{\M^*,h}(s_{k,h}) \\
    = & R_{\M^l,h}(s_{k,h},a_{k,h}) + \mbP_{\M^l,h}V^{*}_{\M^l,h+1}(s_{k,h},a_{k,h}) - R_{\M^*,h}(s_{k,h},a_{k,h}) - \mbP_{\M^*,h}V^{\pi_k}_{\M^*,h+1}(s_{k,h},a_{k,h}) \\
    \leq & \left(R_{\M^l,h}(s_{k,h},a_{k,h}) + \mbP_{\M^l,h}V^*_{\M^l,h+1}(s_{k,h},a_{k,h}) - r_{k,h} - V^*_{\M^l,h}(s_{k,h+1})\right) \\
    & + \left(r_{k,h} - R_{\M^*,h}(s_{k,h},a_{k,h})\right) \\
    & + \left(V^{\pi_k}_{\M^*,h+1}(s_{k,h+1})-\mbP_{\M^*,h}V^{\pi_k}_{\M^*,h+1}(s_{k,h},a_{k,h})\right) \\
    & + \left(V^{*}_{\M^l,h+1}(s_{k,h+1}) - V^{\pi_k}_{\M^*,h+1}(s_{k,h+1})\right).
\end{align*}

Define $\mathcal{F}_{k,h} = \sigma\left(\left\{s_{k',h'},a_{k',h'},r_{k',h'},s_{k',h'+1}\right\}_{1\leq k' \leq k, 1\leq h' \leq H}\cup\left\{s_{k,h^{\prime}}, a_{k,h^{\prime}}, r_{k,h^{\prime}}\right\}_{1 \leq h^{\prime} \leq h-1} \cup\left\{s_{k,h}, a_{k,h}\right\}\right)$. Note that \ref{inq: Martingle 1, fine-tuning} and \ref{inq: Martingle 2, fine-tuning} can be regarded as the summation of martingale differences conditioned on $\{\mathcal{F}_{k,h}\}_{k,h}$. For \ref{inq: Martingle 1, fine-tuning}, by Azuma's inequality, we know that with probability at least $1-\delta/6$,
\begin{align*}
    \sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(r_{k,h} - R_{\M^*,h}(s_{k,h},a_{k,h})\right) \leq&  O(\sqrt{KH \log(1/\delta)}).
\end{align*}

For \ref{inq: Martingle 2, fine-tuning}, we can use Lemma 10 in~\cite{zhang2021model} and a recursive Bellman-type Law of Total Variance (LTV) to provide tight bound. We restate Lemma 10 in \cite{zhang2021model} for completeness.
\begin{lemma}
(Lemma 10 in \cite{zhang2021model}) Let $\left(M_{n}\right)_{n \geq 0}$ be a martingale such that $M_0 = 0$ and $|M_n-M_{n-1}| \leq c$ for some $c > 0$ and any $n \geq 1$. Let $\operatorname{Var}_{n}=\sum_{k=1}^{n} \mathbb{E}\left[\left(M_{k}-M_{k-1}\right)^{2} \mid \mathcal{F}_{k-1}\right]$ for $n \geq 0$, where $\mathcal{F}_{k}=\sigma\left(M_{1}, \ldots, M_{k}\right)$. Then for any positive integer $n$, and any $\epsilon,\sigma > 0$, we have that
\begin{align*}
    \mathbb{P}\left[\left|M_{n}\right| \geq 2 \sqrt{2} \sqrt{\operatorname{Var}_{n} \ln (1 / \delta)}+2 \sqrt{\epsilon \ln (1 / \delta)}+2 c \ln (1 / \delta)\right] \leq 2\left(\log _{2}\left(\frac{n c^{2}}{\epsilon}\right)+1\right) \delta.
\end{align*}
\end{lemma}
Let $M_{k,h} = V^{\pi_k}_{\M^*,h}(s_{k,h})$, $c = H$ and $\epsilon = 1$, we have with probability at least $1-\log(HK)\delta/6$,
\begin{align*}
     &\sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(V^{\pi_k}_{\M^*,h+1}(s_{k,h+1})-\mbP_{\M^*,h}V^{\pi_k}_{\M^*,1}(s_{k,h},a_{k,h})\right) \\
     \leq & c_1 \sum_{k=1}^{K}\sum_{h=1}^{H} \mathbb{V}\left(\mbP_{\M^{*},h,s_{k,h},a_{k,h}}, V^{\pi_k}_{\M^*,h+1}\right) + c_2 \log(1/\delta),
\end{align*}
where $\mathbb{V}\left(\mbP_{\M^{*},h,s_{k,h},a_{k,h}}, V^{\pi_k}_{\M^*,h+1}\right)$ is the one-step variance: $$\mathbb{V}\left(\mbP_{\M^{*},h,s_{k,h},a_{k,h}}, V^{\pi_k}_{\M^*,h+1}\right) = \mathbb{E}\left[\left(V^{\pi_k}_{\M^*,h+1}(s_{k,h+1})-\mbP_{\M^*,h}V^{\pi_k}_{\M^*,1}(s_{k,h},a_{k,h})\right)^2| \mathcal{F}_{k,h}\right].$$
By the law of total variance~\cite{munos1999influence,azar2017minimax,zhang2021reinforcement}, we have $\sum_{h=1}^{H} \mathbb{V}\left(\mbP_{\M^{*},s_{k,h},a_{k,h}}, V^{\pi_k}_{\M^*,h+1}\right) \leq O(1)$. Therefore, we can upper bound \ref{inq: Martingle 2, fine-tuning} as follows:
\begin{align*}
    \sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(V^{\pi_k}_{\M^*,h+1}(s_{k,h+1})-\mbP_{\M^*,h}V^{\pi_k}_{\M^*,1}(s_{k,h},a_{k,h})\right) \leq&  O(\sqrt{K \log(1/\delta)}).
\end{align*}

For \ref{inq: regret part 1, fine-tuning}, this part is exactly $O_{\tau_{l+1}-1, \mathcal{M}^{l}}-\hat{O}_{\tau_{l+1}-1}$ defined in the event $o_{\tau_{l+1}-1,\M_i}$. Note that since $\caM_{l}$ is not eliminated in the episode $\tau_{l+1}-2$, we know that the event $o_{\tau_{l+1}-2, \caM^*}$ does not happen. Therefore, we have
\begin{align*}
    &\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(R_{\M^l,h}(s_{k,h,a_{k,h}}) + \mbP_{\M^l,h}V^*_{\M^l,h+1}(s_{k,h},a_{k,h}) - r_{k,h} - V^*_{\M^l,h}(s_{k,h+1})\right)\\
    \leq &  \sqrt{2H(\tau_{l+1}-1 - \tau_{l}) \log(4K/\delta)} + 1.
\end{align*}

Summing over $l \in [L]$, 
\begin{align*}
     &\sum_{l=1}^{L}\sum_{k = \tau_l}^{\tau_{l+1}-1} \sum_{h=1}^{H} \left(R_{\M^l,h}(s_{k,h,a_{k,h}}) + \mbP_{\M^l,h}V^*_{\M^l,h+1}(s_{k,h},a_{k,h}) - r_{k,h} - V^*_{\M^l,h}(s_{k,h+1})\right) \\
     \leq & \sum_{l=1}^{L}  \sqrt{2H(\tau_{l+1}-1 - \tau_{l}) \log(4K/\delta)} + L \\
     \leq & O\left(\sqrt{HK |\hat{\caU}|\log(4K/\delta) } + |\hat{\caU}|\right).
\end{align*}

Therefore, 
\begin{align*}
    &\sum_{k=1}^{k} \left( V^*_{\caM^*,1}(s_1) - V^{\pi_k}_{\caM^*,1}(s_1)\right) 
    \leq  O\left(\sqrt{HK |\hat{\caU}|\log(4K/\delta) } + |\hat{\caU}|\right) \leq  O\left(\sqrt{HK |{\caU^*}|\log(4K/\delta) } + |{\caU^*}|\right).
\end{align*}
The last inequality is due to $\hat{\caU} \leq |\caU^*|$ by Lemma~\ref{lemma_pretrain}.

Finally, we take expectation over all possible $\M^*$, and we get
\begin{align}
    \label{inq: regret final}
    \reg(K) \leq O\left(\sqrt{HK |{\caU^*}|\log(4K/\delta) } + |{\caU^*}|\right).
\end{align}
\end{proof}

\iffalse
\subsection{Two Illustrating Examples}
\label{appendix: Illustrating Examples}
\paragraph{$\D$ with Small Support} 
When the cardinality of $\Omega$ is small, we have
\begin{align*}
\C(\D) &\leq \sum_{\M_i \in \Omega}p_i \sqrt{ \sum_{\M_j \in \Omega}\log\left(\frac{\left((1-\delta) p_{j}+\delta p_{i}\right)MK}{p_{i}\delta}\right) }\\
&\leq \sum_{\M_i \in \Omega}p_i  \sqrt{M \log \frac{MK}{\delta} + M \log \frac 1 {p_i}}\\
&\leq \sqrt{M \log \frac{MK}{\delta}} + \sum_{\M_i \in \Omega} p_i\sqrt{M\log \frac{1}{p_i}} \leq \sqrt{M \log \frac{M^2 K}{\delta}}
\end{align*}
where the last inequality comes from the concavity of $\log(\cdot)$. 
This implies the upper bound is at most $ \tilde{\mathcal O}(\sqrt{H^2MK})$, successfully remove dependence on $S,A$. 
To the best of our knowledge, this is the first upper bound that achieve this for episodic MDPs.

\paragraph{$\D$ with Large Support}
If $M$ is arbitrarily large and $p_i \leq c_1 e^{-\lambda i}$ for some positive constant $c_1,\lambda$, then $\C(\D) \leq \sqrt{\log \frac{1}{\delta}  \log \frac{K}{\delta}}$ and $|\mathcal U| \leq \log \frac{1}{\delta}$, which gives the upper bound $\tilde {\mathcal O}\sqrt{H^2K}$.
\fi

\iffalse
\subsection{Proof of Corollary~\ref{corollary: misspecified case}}
\label{appendix: corollary proof}
During the proof, we use $\hat{\D}$ and $\{\hat{p}_{i}\}_{i=1}^{M}$ to denote the distribution estimation used as the input of Algorithm~\ref{alg: optimistic posterior fine-tuning}, and we use $\D$ and $\{{p}_{i}\}_{i=1}^{M}$to denote the true prior distribution.
The proof of Corollary~\ref{corollary: misspecified case} almost exactly follows the proof of Theorem~\ref{theorem_useful_restate}. The main difference is two-folds. 

Firstly, we recalculate the probability that $\M^*$ is eliminated from the instance set. From Inq.~\ref{inq: exclusive event} and Inq.~\ref{inq: elimination prob 2}, we know that the probability that $\M^*$ is eliminated from the instance set is upper bounded by
\begin{align*}
    \mathbb{E}_{\M^* \sim {D}} K \sum_{i=1}^{M} \delta_{\mathcal{M}_{i}, \mathcal{M}^{*}} = &  \mathbb{E}_{\M^* \sim {D}} \frac{1}{4M} \sum_{i=1}^{M} \frac{\hat{p}_{i} \delta}{(1-\delta) \hat{p}_{j}+\delta \hat{p}_{i}} \\
    \leq &\mathbb{E}_{\M^* \sim \hat{D}} \frac{1}{4M} \sum_{i=1}^{M} \frac{\hat{p}_{i} \delta}{(1-\delta) \hat{p}_{j}+\delta \hat{p}_{i}} + \epsilon_{TV} \\
    \leq & \delta/2 + \epsilon_{TV},
\end{align*}
where the last inequality is due to Inq.~\ref{inq: elimination prob 2}. Therefore, the failure probability will increase by $\epsilon_{TV}$, which will lead to a $\epsilon_{TV} K$ term in the regret. 

Secondly, the regret calculated in 
\fi
